Complex Urban LiDAR Data Set

This paper presents a Light Detection and Ranging (LiDAR) data set that targets complex urban environments. Urban environments with high-rise buildings and congested traffic pose a significant challenge for many robotics applications. The presented data set is unique in the sense it is able to capture the genuine features of an urban environment (e.g. metropolitan areas, large building complexes and underground parking lots). Data of two-dimensional (2D) and threedimensional (3D) LiDAR, which are typical types of LiDAR sensors, are provided in the data set. The two 16-ray 3D LiDARs are tilted on both sides for maximal coverage. One 2D LiDAR faces backward while the other faces forwards to collect data of roads and buildings, respectively. Raw sensor data from Fiber Optic Gyro (FOG), Inertial Measurement Unit (IMU), and the Global Positioning System (GPS) are presented in a file format for vehicle pose estimation. The pose information of the vehicle estimated at 100 Hz is also presented after applying the graph simultaneous localization and mapping (SLAM) algorithm. For the convenience of development, the file player and data viewer in Robot Operating System (ROS) environment were also released via the web page. The full data sets are available at: http://irap.kaist.ac.kr/dataset. In this website, 3D preview of each data set is provided using WebGL.

==> fig_intro.tex <==
\begin{figure}[!t]
  \centering
  \def\width{0.3\textwidth}%
  %\subfigure[Gangnam]{%
  %  \includegraphics[width=\width]{./figs/gangnam}
  %  \label{fig:gangnam}
  %}
  %\subfigure[Pangyo]{%
  %  \includegraphics[width=\width]{./figs/pangyo}
  %  \label{fig:pangyo}
  %}
  %\subfigure[Buidling Complex]{%
  %  \includegraphics[width=\width]{./figs/apt}
  %  \label{fig:apt}
  %}\\
  \subfigure[Gangnam3D]{%
    \includegraphics[width=\width]{./figs/gangnam3d}
    \label{fig:gangnam3d}
  }
  \subfigure[Pangyo3D]{%
    \includegraphics[width=\width]{./figs/pangyo3d}
    \label{fig:pangyo3d}
  }
  \subfigure[Buidling Complex 3D]{%
    \includegraphics[width=\width]{./figs/apt3d}
    \label{fig:apt3d}
  }\\
  \caption{KAIST urban LiDAR dataset overview.}
  \label{fig:sensors}
\end{figure}

==> fig_sample.tex <==
\begin{figure*}[!t]
  \centering
  \subfigure[Urban structure (3D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp90}
    \label{fig:data_sample1}
  }
  \subfigure[Urban structure (2D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp91}
    \label{fig:data_sample1}
  } 
  \subfigure[Wide road (3D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp81}
    \label{fig:data_sample1}
  }
  \subfigure[Wide road (2D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp80}
    \label{fig:data_sample1}
  }\\  
  \subfigure[Complex building enterance (3D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp51}
    \label{fig:data_sample1}
  }
  \subfigure[Complex building enterance (2D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp50}
    \label{fig:data_sample1}
  } 
  \subfigure[Road markings (3D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp30}
    \label{fig:data_sample1}
  }
  \subfigure[Road markings (2D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp31}
    \label{fig:data_sample1}
  }\\
  \subfigure[High-rise apartment complex (3D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp11}
    \label{fig:data_sample1}
  }
  \subfigure[High-rise apartment complex (2D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp10}
    \label{fig:data_sample1}
  } 
  \subfigure[Underground parking lot (3D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp00}
    \label{fig:data_sample1}
  }
  \subfigure[Underground parking lot (2D \ac{LiDAR})]{%
    \includegraphics[width=0.23\textwidth ,height=0.15\textwidth] {./figs/comp01}
    \label{fig:data_sample1}
  }\\    
  \caption{Point cloud mapping result for comparing 3D \ac{LiDAR} data and 2D \ac{LiDAR} data.}
  \label{fig:sample_pc}
\end{figure*}


==> fig_sensor_coord.tex <==
\begin{figure*}[!t]
  \centering
  \begin{minipage}{0.3\textwidth}
  \subfigure[Top view]{%
    \includegraphics[width=0.95\textwidth] {./figs/sensor_rig_top}
    \label{fig:sensor_rig_top}
  }
  \end{minipage}
  \begin{minipage}{0.34\textwidth}
  \subfigure[Rear view for two 3D LiDARs]{%
   	\includegraphics[width=0.95\textwidth, height=0.5\textwidth] {./figs/vlp-all-back}
   	\label{fig:vlp-all-back}
  }\\
  \subfigure[Side view]{%
   	\includegraphics[width=0.95\textwidth, height=0.5\textwidth] {./figs/sensor_rig_side}
   	\label{fig:side_view}
  }   
  \end{minipage}  
  \begin{minipage}{0.34\textwidth}
  	\subfigure[Side view for two 2D LiDARs]{%
  		\includegraphics[width=0.95\textwidth, height=0.5\textwidth] {./figs/sick_side}
  		\label{fig:sick_side}
  	}\\
  	\subfigure[Rear 2D LiDAR]{%
  		\includegraphics[width=0.46\textwidth, height=0.45\textwidth] {./figs/sick_rear}
  		\label{fig:sick_rear}
  	}\hfil%  
  	\subfigure[Middle 2D LiDAR]{%
          \includegraphics[width=0.46\textwidth, height=0.45\textwidth] {./figs/sick_middle}
          \label{fig:sick_middle}
    }      
  \end{minipage}    
  \caption{Hardware sensor configuration. \subref{fig:sensor_rig_top} Top view and \subref{fig:side_view} side view of the entire sensor system with coordinate frame. Each sensor is mounted on the vehicle, and red, green, and blue arrow indicate x, y, and z coordinate of sensor respectively. \subref{fig:vlp-all-back} Two 3D LiDARs are tilted $45^\circ$ for maximal coverage. \subref{fig:sick_side} Two 2D LiDARs are tilted to face the road and the buildings. \subref{fig:sick_rear} Rear 2D LiDAR is facing down to the road and \subref{fig:sick_middle} middle 2D LiDAR is heading up to detect the building structures. Sensor coordinates are displayed on each sensor figure.}
  \label{fig:sensors}
\end{figure*}

\begin{table*}[!t]
  \centering
  \caption{Specifications of sensors used in sensor system}
  \label{tab:spec}%
  \begin{tabular}{c|ccccccc}%
    Type                   & Manufacturer   & Model         & Description                            		& No.   & Hz    & Accuracy  & Range \\
    \hline
    \textbf{3D LiDAR}      & Velodyne       & VLP-16        & 16 channel Lidar with 360$^\circ$ FOV         & 2     & 20    &      & 100 m\\
    \textbf{2D LiDAR}      & SICK           & LMS-511       & 1 channel 2D LiDAR with 190$^\circ$ FOV  		& 2     & 100   &           & 80 m\\
    \textbf{GPS}           & U-Blox         & EVK-7P        & Consumer level GPS                		& 1     & 10    &  2.5 \unit{m}         &\\
    \textbf{RTK GPS}       & SOKKIA         & GRX 2         & VRS-RTK GPS                            		& 1     & 1     &  H: 10 \unit{mm}, V:15 \unit{mm}   &\\ 
    \textbf{3-axis FOG}    & KVH            & DSP-1760      & Fiber optics gyro (3 axis)             		& 1     & 1000  &  0.05$^\circ$/h  &\\
    \textbf{IMU}           & Xsens          & MTi-300       & consumer level Gyro enhanced AHRS       		& 1     & 200   &  10$^\circ$/h  &\\
    \textbf{Wheel encoder} & RLS            & LM13          & Magnetic rotary encoder                		& 2     & 100   & 4096 (resolution)  &\\
    \hline
  \end{tabular}
\end{table*}


